PatchRefineNet: Improving Binary Segmentation by Incorporating Signals from Optimal Patch-wise Binarization

The purpose of binary segmentation models is to determine which pixels belong to an object of interest (e.g., which pixels in an image are part of roads). The models assign a logit score (i.e., probability) to each pixel and these are converted into predictions by thresholding (i.e., each pixel with logit score $\geq \tau$ is predicted to be part of a road). However, a common phenomenon in current and former state-of-the-art segmentation models is spatial bias -- in some patches, the logit scores are consistently biased upwards and in others they are consistently biased downwards. These biases cause false positives and false negatives in the final predictions. In this paper, we propose PatchRefineNet (PRN), a small network that sits on top of a base segmentation model and learns to correct its patch-specific biases. Across a wide variety of base models, PRN consistently helps them improve mIoU by 2-3\%. One of the key ideas behind PRN is the addition of a novel supervision signal during training. Given the logit scores produced by the base segmentation model, each pixel is given a pseudo-label that is obtained by optimally thresholding the logit scores in each image patch. Incorporating these pseudo-labels into the loss function of PRN helps correct systematic biases and reduce false positives/negatives. Although we mainly focus on binary segmentation, we also show how PRN can be extended to saliency detection and few-shot segmentation. We also discuss how the ideas can be extended to multiclass segmentation.

==> related_work.tex <==
\section{Related Work}\label{sec:related_work}
\noindent\textbf{Applications using Binary Annotation.}\\
 Binary annotation is a popular annotation strategy, currently being extensively used in applications such as geo-spatial \cite{nagendra2022constructing, zhou2018d, zheng2020foreground, alirezaie2019semantic} and medical \cite{pham2000survey, jha2020kvasir, zhou2018unet++} segmentation. Furthermore, it is used in Saliency detection \cite{zhao2019pyramid, hou2007saliency, goferman2011context, wang2017learning}, and Few-shot segmentation \cite{li2020fss, li2022language}.  State-of-the-art network architectures \cite{chen2017rethinking, chen2018encoder, sun2019high, zhao2017pyramid, yuan2018ocnet, zhang2019co, fu2019dual, huang2019interlaced, chen2017deeplab, chen2016attention, farabet2012learning, he2004multiscale, nagendra2017comparison} designed for these applications exhibit spatial biases that limit the accuracy of the resulting binarized predictions. \ours is designed to eliminate such spatial biases, thus improving binary segmentation performance in these applications. \\\\
\noindent\textbf{Segmentation Network Architectures.} \\
Most of the existing works address semantic segmentation through (i) improving boundary quality \cite{chen2017rethinking, chen2018encoder, sun2019high}, (ii) constructing reliable context information by increasing field-of-view \cite{zhao2017pyramid, yuan2018ocnet, zhang2019co, fu2019dual, huang2019interlaced, chen2017deeplab, chen2016attention, farabet2012learning, he2004multiscale, nagendra2017comparison}, (iii) increasing resolution of feature maps \cite{chen2017rethinking, chen2018encoder, sun2019high} and (iv) refining semantic segmentation maps as a post-processing step \cite{cheng2020cascadepsp, chen2014semantic, yuan2020segfix}. In this paper, we design PRN  following the fourth line of work.  Design of segmentation architectures typically have the following components for improving performance -- Feature pyramid methods \cite{liu2015parsenet, he2015spatial,cheng2020cascadepsp, funk2018learning} for spatially pooling feature maps of different receptive fields, dilated convolutions \cite{yu2015multi} for increasing field-of-view,  encoder-decoder models \cite{badrinarayanan2017segnet, chen2018encoder, li2018pyramid, liu2019auto,liu2018path,noh2015learning,ronneberger2015u, liu2021new, pei2021utilizing, pei2020cloud} for reducing spatial resolution to capture global semantics followed by a decoder for restoring spatial resolution. Skip connections \cite{ronneberger2015u, cheng2020cascadepsp, nagendra2020efficient} are added to recover lost spatial information in deeper layers.  Self-attention \cite{oktay2018attention, huang2019interlaced, ye2019cross, zhou2021self} is used to highlight salient features from spatial-information-rich skip connections and feature maps from deeper layers, where attention coefficients are more sensitive to local regions. Recently, the Vision Transformer (ViT) \cite{arnab2021vivit} introduced a convolution-free transformer architecture for image classification with patch tokens and multi-head self-attention \cite{vaswani2017attention}. However, the caveat is they require extensive training data. Further, multi-scale context aggregation \cite{chen2014semantic, chen2016attention, xia2016zoom, hariharan2015hypercolumns} has proven to be efficient for integrating high-level and low-level features. Since \ours is a post-processing scheme, it must be light-weight with memory-efficient training and quick convergence. Inspired by previous network designs and taking the constraints of \ours design into consideration, we make \ours to be a residual encoder-decoder with pyramid pooling for context aggregation, skip connections for sharper boundaries, self-attention for highlighting important local regions, and multi-scale context aggregation with simultaneously trainable global \& local branches.
\\\\
\noindent\textbf{Segmentation Refinement. }\\ Despite large improvements in network architectures that employ the above-mentioned strategies, existing methods still show poor boundary adherence and loss of high-resolution fine structures due to spatial biases in predicted logit maps \cite{jha2019resunet++, zhou2018d, zhao2019pyramid, li2020fss, nagendra2022constructing}. Post-processing refinement strategies have been previously use to improve segmentation performance. Unsupervised probabilistic frameworks such as Conditional Random Fields \cite{chen2017deeplab, chen2014semantic, zheng2015conditional} or region growing \cite{dias2020probabilistic, dias2018semantic} adhere to local semantics without fully leveraging global information. There are methods that exploit only boundary information \cite{yuan2020segfix}. Some methods use cascading and multi-scale context aggregation to generate for increasing contextual semantics \cite{cheng2020cascadepsp}. In this paper, we compare \ours with CascadePSP \cite{cheng2020cascadepsp} and DenseCRF \cite{zheng2015conditional}. DenseCRF is limited to extracting only local semantics from neighborhood pixels. CascadePSP is designed specifically for generating high-resolution maps. It uses cascaded global and local steps for iterative refinement, unlike \ours which is a one-pass refinement module. The local step in \cite{cheng2020cascadepsp} is memory-intensive for producing finer segmentation maps, while memory usage of \ours is constant for all patch sizes. %\textbf{Adaptive Thresholding. } This work should not be confused with \emph{adaptive thresholding} \cite{bradley2007adaptive}, which is a framework for producing binary images based on a threshold that varies with the illumination in different parts of an image.


